Counting $SL(2,\mathbb{C})$ connections on Seifert-fibered spaces

We study the $SL(2, \mathbb{C})$ character variety of a Seifert-fibered homology $3$-sphere from the point of view of gauge theory. Namely, we introduce a class of perturbations of the $SL(2,\mathbb{C})$ Chern--Simons functional and prove a localisation result: the perturbed critical points either approach a compact subset of the $SL(2, \mathbb{C})$ character variety or else `escape to infinity'. Furthermore, the Euler characteristic and Poincar\'e polynomial of the stable locus of the character variety are obtained by suitably counting the localising critical points. As an application, we obtain formulae for the Euler characteristic and Poincar\'e polynomial of the stable locus of the $SL(2, \mathbb{C})$ character variety of a Seifert-fibered homology $3$-sphere. In particular, we prove that the Euler characteristic equals the Milnor number (divided by four) of any weighted-homogeneous isolated complete intersection singularity whose link is the given $3$-manifold.

==> deleted.tex <==
%Let $X \subset \mathbb{C}^{k+2}$ be a \textit{weighted-homogeneous complete intersection} of $\dim_{\mathbb{C}} X = 2$ and with an isolated singular point at $0 \in X$, with degrees $d = (d_1 , \ldots , d_k )$ and weights $(w_1 , \ldots , w_{k+2})$. This means that 


Let $f : \mathbb{C}^{n+1}\rightarrow \mathbb{C}$ be a polynomial with an \textit{isolated singularity} at $0 \in \mathbb{C}^{n+1}$ and $f(0) = 0$. The vanishing locus $X = V(f)$ is an $n$-dimensional \textit{isolated hypersurface singularity} (abbreviated to IHS). %, and let $X = V(f) \subset \mathbb{C}^{n+1}$ be  the associated \textit{isolated hypersurface singularity}. 
The local structure near the singular point of $f$ can be probed through the \textit{Milnor fibration} of $f$, which is the family of smooth compact $2n$-manifolds with boundary (called \textit{Milnor fibers}) given as the fibers of the $C^\infty$ fiber-bundle
\begin{align}
f^{-1}(B_{\delta}(\mathbb{C},0)\setminus 0) \cap B_{\epsilon}(\mathbb{C}^{n+1},0) \xrightarrow{f} B_{\delta}(\mathbb{C},0) \setminus 0 \label{milnor1}
\end{align}
where $0 < \delta \ll \epsilon \ll 1$. A Milnor fiber $M$ has the homotopy type of a wedge of $\mu$ $n$-spheres, where $\mu$ is the \textit{Milnor number} of $f$ at $0 \in \mathbb{C}^{n+1}$. \JL{We are interested in  topological properties of the monodromy $\psi$ of the Milnor fibration (\ref{milnor1}). Since the work of Milnor \cite{milnor,milnorbrieskorn} and Brieskorn \cite{brieskorn,brieskornADE}, this has been a central topic in the study of singularities by topological methods. While most classical researches study the induced auotomorphism $\psi_*$ on $H_{n}(M;\mathbb{Z})$, considerably less is known about the \textit{monodromy diffeomorphism} as an element in the smooth mapping class group $\pi_0(\diff(M,\partial))$. This is especially the case when $n=2$. This motivates us to use gauge theory to extract additional information from the monodromy diffeomorphism.}

We will focus on the case of an IHS defined by a \textit{weighted-homogeneous} polynomial, meaning that there exist positive integers $w_1 , \ldots , w_{n+1}, d$ such that $f(t^{w_1} x_1 , \ldots , t^{w_{n+1}}x_{n+1} ) = t^{d}f(x_1 , \ldots , x_{n+1})$ for all $t \in \mathbb{C}$, such as the Brieskorn--Pham polynomials $f = \sum_{j = 1}^{n+1} (x_j )^{a_j}$ for $a_j \in \mathbb{Z}_{\geq 2}$. %The weighted-homogeneous IHS's a precisely the affine quasicones on quasismooth hypersurfaces in weighted projective spaces \cite{dolgachev} 
The monodromy of such singularities has been extensively studied using algebraic techniques \cite{}. Our main result is the following

%(and without loss of generality, the $w_1 , \ldots , w_n$ have no common factors).


\begin{theorem}\label{theorem:singularities}
If $X = V(f)$ is a weighted-homogeneous IHS of dimension $n = 2$ whose link is a rational homology 3-sphere and $X$ is not a rational double-point singularity, then the monodromy $\psi$ of the Milnor fibration of $f$ has infinite order in the smooth mapping class group $\pi_0 (\mathrm{Diff}(M, \partial ))$.
\end{theorem}


We recall that a \textit{rational double-point} is a $2$-dimensional IHS $X$ whose \textit{geometric genus} $p_g (X) = 0$ (these are precisely the \textit{ADE singularities}, which are all weighted-homogeneous). Brieskorn's Theorem on the simultaneous resolution of rational double-points \cite{brieskornADE} shows that the monodromy $\psi$ of the Milnor fibration of a rational double-point has finite order in $\pi_0 ( \mathrm{Diff}(M, \partial )$) (namely, the order is the Coxeter number of the associated Weyl group). Thus, Theorem \ref{theorem:singularities} provides a \textit{differential-topological explanation} to the non-existence of simultaneous resolutions when $p_g > 0$.
Under the additional hypothesis $p_g(X) = 1$, the above result was established in previous work of the authors \cite[Corollary 1.2]{KLMME} using very different techniques that could not handle the case $p_g > 1$. Theorem \ref{theorem:singularities} proves \cite[Conjecture 1.3]{KLMME}.

Theorem \ref{theorem:singularities} stands in sharp contrast with the higher dimensional case. For example, if instead $X$ is an $n$-dimensional weighted-homogeneous IHS whose link is an integral homology $(2n-1)$-sphere and $n > 4$ then the monodromy $\psi$ has finite order in $\pi_0 (  \mathrm{Diff}(M, \partial ))$ \cite[Proposition 2.22]{KLMME}. For a weighted-homogeneous IHS $X$ of any dimension $n > 1$, the action of the monodromy on the middle homology $H_2 (M )$ has finite order \cite{milnor}. Furthermore, if $n = 2$ and the link is a rational homology $3$-sphere, this implies, by a result of Orson--Powell \cite{orson-powell}, that the monodromy has finite order in the \textit{topological} mapping class group $\pi_0 ( \mathrm{Homeo}(M, \partial)  )$. Dropping the weighted-homogeneous assumption, we propose the following

\begin{conjecture}
\label{conjecture, not only weighted homogeneous}
If $X = V(f)$ is an IHS of dimension $n =2$ and $X$ is not a rational double point singularity, then the monodromy $\psi$ of the Milnor fibration of $f$ has infinite order in the smooth mapping class group $\pi_0 (\mathrm{Diff}(M, \partial ))$.
\end{conjecture}




Theorem \ref{theorem:singularities} has remarkable implications regarding the \textit{monodromy group} of a $n = 2$-dimensional weighted-homogeneous IHS $X = V(f)$, which we now explain (see \S \ref{section:singularities} for further details). One can `Morsify' $f$ by adding in linear terms, i.e. consider $\widetilde{f} = f + \sum_{i =1}^3 a_i x_i$ for a generic choice of coefficients $a_i \in \mathbb{C}$. The subgroup $\Theta (X) \subset \pi_0 ( \mathrm{Diff}(M, \partial) )$ generated by the reflections on the vanishing $2$-spheres of the Morse function $\widetilde{f}$, for some choice of vanishing paths,
does not depend on the choices made. We refer to $\Theta(X)$ as the `geometric' monodromy group of $X$, whereas the `classical' monodromy group $\Theta_h (X)$ is defined as the image of $\Theta(X)$ under the canonical map $h:  \pi_0 ( \mathrm{Diff}(M, \partial ) ) \rightarrow \mathrm{Aut}(H_2 (M, \mathbb{Z} ) )$ with target the automorphism group of the intersection pairing on the middle-degree homology. When $X$ is a rational double-point then the comparison map $\Theta (X ) \rightarrow \Theta_h (X) $ is an isomorphism (and both groups are isomorphic to a suitable Weyl group), which follows from Brieskorn's Theorem. In contrast, Theorem \ref{theorem:singularities} implies the following

\begin{corollary}\label{cor:monodromygroup}
If $X = V(f)$ is a weighted-homogeneous IHS of dimension $n = 2$ whose link is a rational homology 3-sphere and $X$ is not a rational double-point singularity, then the kernel of the comparison map $\Theta (X ) \rightarrow \Theta_h (X)$ contains a $\mathbb{Z}$ subgroup. \JL{In particular, the comparison map is not an isomorphism.}
\end{corollary}

\JL{Theorem \ref{thm: main} can be generalized to equivariant smoothings of weighted-homogeneous isolated surface singularities which are not necessarily hypersurfaces. And it can also be generalized to  certain singularities which are not weighted homogeneous. We refer to \S \ref{section:singularities} for these generalizations and further discussions.}

%various generalizations of the above results to isolated surface singularities which are not necessarily hypersurfaces. 

%For further discussion pertaining these results we refer to \S \ref{section:singularities} below.



%\JM{Should we include here the Conjecture about infinite-order monodromy for arbitrary singularities, not just the weighted ones?}\JL{Yeah, let's do that.}





\begin{lemma} There exists a family spin-c structure $\fs_{\widetilde{M}_{n}}$ that restricts to $\fs_{M}$ on each fiber.
\end{lemma}
\begin{proof} Let $\operatorname{Aut}(M,\fs_{M})$ be the group of automorphism of the spinor bundle. Then finding a family spin-c structure on $\widetilde{M}_{n}$ amounts to solving the lifting problem 
\[
\xymatrix{& \operatorname{BAut}(M,\fs_{M})\ar[d]\\
BG_{n}\ar[r]\ar@{-->}[ru] & \bdiff(M)}
\]
Note the fibration 
\[
\operatorname{BMap}(M,S^{1})\to \operatorname{BAut}(M,\fs_{M})\to \bdiff(M)
\]
So the obstruction $o_{i}$ of this lifting problem is in 
\[
H^{i}(BG_{n};\pi_{i-1}(\operatorname{BMap}(M,S^{1})))=H^{i}(BG_{n};H^{1}(S^{i-2}\times M;\mathbb{Z}))
\]
For $i=2$, this group is $H^{2}(BG_{n};H^{1}(M;\mathbb{Z}))=0$. For $i=3$, this group is \[H^{3}(BG_{n}; H^{1}(M\times S^{1};\mathbb{Z}))=H^{3}(BG_{n}; \mathbb{Z})=0.\] For other values of $i$, this group is obviously zero.
\end{proof}


We apply the coBorel cohomology and the Tate cohomology to the relative Bauer-Furuta invariant (\ref{eq: Bauer-Furuta}) and get the induced maps 
 that fit into the commutative diagram
\[
\xymatrix{ tH^*_{S^1}(\SWF(Y,\fs);\F)
 \ar[rr]^-{\overline{HM}^*(M,\fs_{M})} \ar[d] &&tH^*_{S^1}(\Pic(M,\fs_{M});\F)\ar[d]\\
cH^*_{S^1}(\SWF(Y,\fs);\F) \ar[rr]^-{\widehat{HM}^*(M,\fs_{M})} & & cH^*_{S^1}(\Pic(M,\fs_{M});\F)}
\]
Let $\beta\in H^{b_{1}(M)}(\Pic(M,\fs_{M});\F)$ be the generator 


Note that the relative Bauer-Furuta invariant of $M$ is a stable, $S^1$-equivariant map  \[ \baf(M,\fs_{M}):S^{\frac{c^2_{1}(\fs_{M})-\sigma(M)}{8}\mathbb{C}}\to S^{b^{+}}\wedge \SWF(Y) . \] Applying the co-Borel cohomology and the Tata cohomology functor, we obtain the maps $\widehat{HM}^*(M,\fs_{M})$ and $\overline{HM}^*(M,\fs_{M})$ that fit into the commutative diagram
\[
\xymatrix{ \overline{HM}^*(Y,\fs;\F)
 \ar[rr]^{\overline{HM}^*(M,\fs_{M})} \ar[d] &&\F[U^{-1},U]\ar[d]\\
\widehat{HM}^*(Y,\fs;\F) \ar[rr]^{\widehat{HM}^*(M,\fs_{M})} & & \F[U^{-1},U]/(U)}
\]
Since $b^+(M)>0$, the restriction of $\baf$ to $S^{1}$-fixed points is trivial. So the induced map $\overline{HM}^*(Y,\fs;\F)$ on Tate cohomology is trivial. Therefore, $\widehat{HM}^*(M,\fs_{M})$ induced a mixed map
\[
\overrightarrow{HM}^*(M,\fs_{M}): HM_{\reduced}^*(Y,\fs;\F)\to \F[U^{-1},U]/(U)
\]
Here we treat $HM_{\reduced}^*(Y,\fs;\F)$ as the cokernel of 
$\overline{HM}^*(Y,\fs;\F)\to \widehat{HM}^*(Y,\fs;\F)$ through the exact triangle relating $\widecheck{HM},\widehat{HM}$ and $\overline{HM}$.
\begin{lemma} There exists $\alpha \in HM_{\reduced}^*(Y,\fs;\F)$ such that 
\[\overrightarrow{HM}^*(M,\fs_{M})(\alpha)=1\in \mathbb{F}[U^{-1},U]/(U).\]    
\end{lemma}
\begin{proof}
There exists a (simply-connected?) symplectic cap $(W,\fs_{W})$ of $(Y,\xi)$ such that $b^{+}(W)>0$. By applying Borel cohomology to the relative Bauer-Furuta invariant of $(W,\fs_{W})$, we obtain a map 
\[
\widecheck{HM}^{*}(W,\fs_{W}): \F[U]\to \widecheck{HM}^*(Y,\fs;\F)
\]
Agian, since $b^{+}(W)>0$, the image of this map belongs to $HM^*_{\reduced}(Y,\fs)$. We let \[\alpha= \widecheck{HM}^{*}(W,\fs_{W})(1).\] Then the gluing theorem for Bauer-Furuta invariant \cite{Manolescugluing} (together with the fact that Bauer-Furuta invariant of closed 4-manifolds recovers the Seiberg-Witten invariant) implies that 
\[
\overrightarrow{HM}^*(M,\fs_{M})(\alpha)= \operatorname{SW}(M\cup W, \fs_{M}\cup \fs_{W})=1.
\]
\end{proof}


\begin{equation}\label{eq: Bauer-Furuta}
\Bafu(M,\fs_{M}): S^{-n(Y,g,\fs)\mathbb{C}}\wedge \Th(D)\to S^{b^{+}(M)}\wedge \SWF(Y,\fs)    
\end{equation}

Here $\Th(D)$ denotes the Thom spectrum of the index bundle $\operatorname{Ind}(D)$ over  $\Pic(M,\fs_{M})$ of the Dirac operator, with the Atiyah-Partodi-Singer boundary condition. And we do a formal desuspension on 
$\Th(D)$ by $n(Y,g,\fs)$ copies of $\mathbb{C}$, where
\[n(Y,g,\fs):=\operatorname{ind}_{\mathbb{C}}(D)-\frac{c^2_{1}(\fs_{M})-\sigma(M)}{8}\in \mathbb{Q}\]
is the index-theoretic correction term. One can apply the coBorel cohomology and the Tate cohomology to (\ref{eq: Bauer-Furuta}) and obtain maps induced by cobordism that fit into the commutative daigram
\[ \xymatrix{ tH^*_{S^1}(\SWF(Y,\fs);\F)  \ar[rr]^-{\overline{HM}^*(M,\fs_{M})} \ar[d]^{q_{Y}} &&tH^*_{S^1}(\Th(D);\F)\ar[d]^{q}\\ cH^*_{S^1}(\SWF(Y,\fs);\F) \ar[rr]^-{\widehat{HM}^*(M,\fs_{M})} & & cH^*_{S^1}( \Th(D);\F)} \].
By the Thom isomorphism theorem, we have 
\[
tH^*_{S^1}(\Th(D);\F)\cong tH^*_{S^1}(\Pic(M,\fs_{M});\F)\cong H^*(\Pic(M,\fs_{M});\F)\otimes_{\F}\F[U,U^{-1}]
\]
and 
\[
cH^*_{S^1}(\Th(D);\F)\cong cH^*_{S^1}(\Pic(M,\fs_{M});\F)\cong H^*(\Pic(M,\fs_{M});\F)\otimes_{\F}\F[U,U^{-1}]/(U)
\]
Under these isomorphisms, $q$ is just the quotient map. 

Also note that the map $\overline{HM}^*(M,\fs_{M})$ is determined by the restriction of $\Bafu(M,\fs_{M})$ to the $S^1$-geometric fixed point spectra. This restriction equals the composition 
\[
\Pic(M,\fs_{M})_{+}\to S^0\to S^{b^{+}(M)}.
\]
so is null-homotopic if $b^{+}(M)>0$. In this case, the map $\widehat{HM}^*(M,\fs_{M})$ induces a map 
\[
\overrightarrow{HM}^*(M,\fs_{M}): HM^*_{\reduced}(Y,\fs_{Y};\F)\to H^*(\Pic(M,\fs_{M});\F)\otimes_{\F}\F[U,U^{-1}]/(U)
\]
Here $HM^*_{\reduced}(Y,\fs_{Y};\F):=\coker q_{Y}$.

\begin{lemma}\label{lem：HM-red surjective} The induced map 
$i^*: HM^{*}_{\reduced,G}(Y,\fs;\F)\to HM^{*}_{\reduced}(Y,\fs;\F)$
is surjective.
\end{lemma}
\begin{proof}
A spectral from the nonequivariant monopole Floer cohomology to the equivariant monopole Floer cohomology is established in \cite{Baraglia2024equivariant}, which arises as the Serre spectral sequence for (\ref{eq: SWF fibration}). If we use integer coefficients, then the $E_{2}$-page is given by 
\[
E^{p,q}_{2}=H^{p}(BG;\widecheck{HM}^{q}(Y,\fs;\mathbb{Z})),\quad p\in \mathbb{N}, q\in \mathbb{Q},
\]
and the spectral sequence converges to $\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{Z})$. Since the generator of the $G$-action on $Y$ is isotopic to the identity, the monodromy action of (\ref{eq: SWF fibration}) on $\widecheck{HM}^{*}(Y,\fs;\mathbb{Z})$ is trivial. Moreover, $\widecheck{HM}^{*}(Y,\fs;\mathbb{Z})$ can be computed by the graded roots algorithm \cite{Nemethi11}. In particular, the two sumannds of the decomposition
\[
\widecheck{HM}^{*}(Y,\fs;\mathbb{Z})\cong \mathbb{Z}[U]_{d(Y,\fs)}\oplus HM^{*}_{\reduced}(Y,\fs;\mathbb{Z}),
\]
which are supported in different relative $\mathbb{Z}/2$-grading gradings. \HK{Here $d(Y,\fs)$ denotes the Heegaard Floer correction term \cite{}.} This decomposition induces a decomposition $E^{*,*}_{2}=V_{1}\oplus V_{2}$, where 
\[
V_{1}=(\mathbb{Z}[U]_{d(Y,\fs)}\otimes_{\mathbb{Z}} H^{*}(BG;\mathbb{Z}))
\]
and 
\[
V_{2}=(HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})\otimes_{\mathbb{Z}}H^{*}(BG;\mathbb{Z}))).
\]
 Note that $V_2$ is $U$-torsion, while $V_1$ is $U$-torsion free. So $V_2$ cannot support a differential to $V_1$. On the other hand, since $HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})$ and $H^{*}(BG;\mathbb{Z})$ are both supported in a single $\mathbb{Z}/2$-grading, $V_2$ is also supported in a single $\mathbb{Z}/2$-grading. Hence there cannot be any differential from $V_2$ to itself. We have proved that  $V_2$ does not support any higher differentials. Also note that the differential $d^{k}$ sends $E^{k}_{p,q}$ to $E^{k}_{p+k,q-k+1}$. So 
\[HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})\otimes 1\subset E^{2}_{0,*} 
\]
cannot be hit by $d^{k}$. To this end, we see that $HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})\otimes 1$ survives to the $E_\infty$-page. This implies that  
$i^*: HM^{*}_{\reduced,G}(Y,\fs;\mathbb{Z})\to HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})$
is surjective. \JL{A gap here. Will fix.} Since the change-of-coefficient map 
\[
HM^{*}_{\reduced}(Y,\fs;\mathbb{Z})\to HM^{*}_{\reduced}(Y,\fs;\F)
\]
is also surjective, the proof is finished.
\end{proof}


For $p\gg 0$, we have $S^{-1}HM^{*}_{G,red}(Y,\fs;\mathbb{F})=0$.    
\end{lemma}
\begin{proof}
The localization theorem in equivariant cohomology \cite[III, Theorem 3.8]{tomDieck}, applied to $\SWF(Y,\mathfrak{s})$, implies that
\HK{
\[S^{-1}\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{F})\cong S^{-1} \tilde{H}^{*+2n(Y,\fs,g)}_{G\times S^1}(\SWF(Y,\fs,g)^{G})).\]
}
Here $\SWF(Y,\fs,g)^{G}$ denotes the geometric fixed point of $\SWF(Y,\fs,g)$. On the other hand, it is proved in \cite{LidmanManolescu}) that 
\[\SWF(Y,\fs,g)^{G}\simeq \SWF(Y/G,\fs/G,g/G).\] So we have the isomorphism 
\[S^{-1}\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{F})\cong \widecheck{HM}^{*}(Y/G,\fs/G;\mathbb{F})\otimes_{\F} \F[S,S^{-1},R]/(R^2)\]
as relative $\mathbb{Z}$-graded modules. On the other hand, we have 
\[
HM_{\reduced}(Y/G,\fs_0;\mathbb{F})=0
\]
when $p\gg 0$ \cite[Proposition 6.2]{baraglia2024brieskorn}. Here $\fs_0$ denotes the canonical spin-c structure on $Y/G$. So $Y/G$ must be an $L$-space because otherwise $\fs_0$ would support a taut foliation \cite{lisca-stipsicz}, \JM{and thus we would have $HM_{red}(Y/G , \mathfrak{s}_0 ; \mathbb{F} ) \neq 0$ by \cite{monolens}}. So we have
\[
S^{-1}\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{F})\cong \F[U,S,S^{-1},R]/(R^2).
\]
This implies the exact sequence
\[
0\to S^{-1}\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{F})\to S^{-1}U^{-1}\widecheck{HM}^{*}_{G}(Y,\fs;\mathbb{F})
\]
Since the localization functor $S^{-1}(-)$ is exact, we see that $S^{-1}HM^{*}_{G,red}(Y,\fs;\mathbb{F})=0$.
\end{proof}



After a suitable desuspension of (\ref{eq: unsuspended relative BF}), one obtains the relative Bauer-Furuta invariant for the family $\widetilde{M}/B$. This is an $S^1$-equivariant stable homotopy class
 \[
\FBafu(\widetilde{M}/B,\fs_{M}): S^{-n(Y,\fs_{Y},g)\mathbb{C}}\wedge \Th(\widetilde{D}^+)\to \SWF(\widetilde{Y}/B,\fs_{Y},g) \wedge (\R^{b^+(W)})^+.
\]
\HK{(HK: $(\R^{b^+(W)})^+$ is added at the right-hand side. Also, dependence on $g$ is added for SWF.)}
The notations are explained as follows:
\begin{itemize}
    \item $\SWF(\widetilde{Y}/B,\fs_{Y},g)$ denotes the $S^{1}$-equivariant CW spectra obtained as follows. \HK{First, we have a family $\widetilde{\SWF}(\widetilde{Y}/B,\fs_{Y},g) :=(\SWF(Y,\fs_{Y},g)\wedge E_{+})/G$ over $B$. Each fiber of this family has a base point, so we obtain a section $s : B \to \widetilde{\SWF}(\widetilde{Y}/B,\fs_{Y},g)$ by collecting such points. Now $\SWF(\widetilde{Y}/B,\fs_{Y})$ is defined as the quotient
    \[
    \SWF(\widetilde{Y}/B,\fs_{Y}) := \widetilde{\SWF}(\widetilde{Y}/B,\fs_{Y},g)/s(B).
    \]}
    
    \item $\Th(\widetilde{D}^+)$ denotes the Thom spectra for the index bundle of the family Dirac operator over $\Pic(\widetilde{M},\fs_{M})$.
    \item $S^{-n(Y,\fs_{Y},g)\mathbb{C}}\wedge-$ denotes the formal desuspension by $n(Y,\fs_{Y},g)$ copies of $\mathbb{C}$ \HK{and $n(Y,\fs_Y,g)$ is the quantity defined in \eqref{eq: n(Y,g)}.}
%where 
%\[n(Y,g,\fs):=\operatorname{ind}_{\mathbb{C}}(D^+)-\frac{c^2_{1}(\fs_{M})-\sigma(M)}{8}\in \mathbb{Q}\]
%is the index-theoretic correction term. 
\end{itemize} 
Next, we apply \HK{reduced} Tate cohomology $t\tilde{H}^{*}_{S^1}(-;\F)$ and coBorel cohomology $c\tilde{H}^{*}_{S^1}(-;\F)$ on $\FBafu(\widetilde{M}/B,\fs_{M})$. \HK{(HK: I put tilde for based spaces here and below.)}
\HK{We use the notation 
\[
\widececk{HM}^*(-) = \tilde{H}^{*}_{S^1}(-;\F),\quad
\widehat{HM}^*(-) = c\tilde{H}^{*}_{S^1}(-;\F),\quad
\overline{HM}^*(-) = t\tilde{H}^{*}_{S^1}(-;\F)
\]
for the cobordism maps, for the analogy with monopole Floer homology.}
The induced maps fit the commutative diagram
\[ \xymatrix{ t\tilde{H}^*_{S^1}(\SWF(\widetilde{Y}/B,\fs_{Y});\F)  \ar[rr]^-{\overline{HM}^*(\widetilde{M}/B,\fs_{M})} \ar[d] &&t\tilde{H}^*_{S^1}(\Th(\widetilde{D}^+);\F)\ar[d]\\ c\tilde{H}^*_{S^1}(\SWF(\widetilde{Y}/B,\fs_{Y});\F) \ar[rr]^-{\widehat{HM}^*(\widetilde{M}/B,\fs_{M})} & & c\tilde{H}^*_{S^1}( \Th(\widetilde{D}^+);\F)}. \]
By the Thom isomorphism theorem, after a grading shift, we have the isomorphism 
\[
c\tilde{H}^*_{S^1}( \Th(\widetilde{D}^+);\F)\cong cH^*_{S^1}(\Pic(\widetilde{M}/B,\fs_{M});\F).
\]
Since the $S^1$-action on $\Pic(\widetilde{M}/B,\fs_{M})$ is trivial, we have the isomorphism 
\[
cH^*_{S^1}(\Pic(\widetilde{M}/B,\fs_{M});\F)\cong H^{*}(\Pic(\widetilde{M}/B,\fs_{M});\F)\otimes_{\F}R,
\]
where $R=cH^{*}_{S^1}(\text{point})=\F[U,U^{-1}]/(U)$.

As the induced map on the Tate cohomology, $\overline{HM}^*(\widetilde{M}/B,\fs_{M})$ is completely determined by $\FBafu(\widetilde{M}/B,\fs_{M})^{S^1}$, the restriction of $\FBafu(\widetilde{M}/B,\fs_{M})$ to the $S^1$-geometric fixed point spectra. By the construction sketched above, $\FBafu(\widetilde{M}/B,\fs_{M})^{S^1}$ equals the composition 
\[
\Pic(\widetilde{M}/B,\fs_{M})_{+}\to S^0\to S^{b^{+}(M)}.
\]
Now suppose $b^{+}(M)>0$, then $\FBafu(\widetilde{M}/B,\fs_{M})^{S^1}$ is null-homotopic. Hence $\overline{HM}^*(\widetilde{M}/B,\fs_{M})=0$. As a result, we get a well-defined mixed map  
\[
\overrightarrow{HM}^*(\widetilde{M}/B,\fs_{M}): HM^*_{\reduced}(\widetilde{Y}/B,\fs_{Y};\F)\to H^*(\Pic(\widetilde{M}/B,\fs_{M});\F)\otimes_{\F}R,
\]
where 
\[
HM^*_{\reduced}(\widetilde{Y}/B,\fs_{Y};\F):=\coker(t\tilde{H}^*_{S^1}(\SWF(\widetilde{Y}/B,\fs_{Y});\F)\to c\tilde{H}^*_{S^1}(\SWF(\widetilde{Y}/B,\fs_{Y});\F)).
\]
This mixed map is a map of $H^*(B;\F)$-modules because (\ref{eq: approximated SW with restriction map}) covers the identity map of $B$. It has a naturality property: Let $\widetilde{M}'/B'$ (resp. $\widetilde{Y}'/B'$) be the pull back of $\widetilde{M}/B$ (resp. $\widetilde{Y}/B$) via a continuous map $i:B'\to B$. Then we have a induced bundle map $j: \Pic(\widetilde{M}'/B')\to\Pic(\widetilde{M}/B)$ that covers $i$. And the following diagram commutes




\begin{proposition}\label{prop: alpha exist}
There exists $\alpha\in HM^*_{\reduced}(Y,\fs_{Y};\F)$ such 
\begin{equation}\label{eq: alpha pair with pic}
\langle \overrightarrow{HM}^*(M,\fs_{M})(\alpha),[\Pic(M,\fs_{M})]\rangle =1\in R.    
\end{equation}
\end{proposition}
\begin{proof}
By \cite{EMM}, there exists a simply-connected  symplectic cap $(W,\fs_{W})$ of $(Y,\xi)$ such that $b^{+}(W)>b_{1}(M)+1$. By applying Borel cohomology to the relative Bauer-Furuta invariant $\Bafu(W,\fs_{W})$, we obtain a map 
\[
\widecheck{HM}^{*}(W,\fs_{W}): \F[U]\to \widecheck{HM}^*(Y,\fs_Y;\F).
\]
Since $b^{+}(W)>0$, the image of this map belongs to $HM^*_{\reduced}(Y,\fs_Y)$. We let \[\alpha= \widecheck{HM}^{*}(W,\fs_{W})(1).\] 
Consider the closed manifold $M\cup W$, which is symplectic with the canonical spin-c structure $\fs_{M}\cup \fs_{W}$. By Taubes' theorem \cite{Taubes94}, we have 
\[
\operatorname{SW}(M\cup W,\fs_{M}\cup \fs_{W} )=1.
\]
Since $b^{+}(M\cup W)>b_{1}(M\cup W)+1$, this Seiberg-Witten invariant can also be extracted from the Bauer-Furuta invariant $\Bafu(M\cup W,\fs_{M}\cup \fs_{W})$ \cite[Proposition 3.3]{BauerFurutaI}. On the other hand, the gluing theorem for Bauer-Furuta invariant \cite{Manolescugluing} allows us to recover $\Bafu(M\cup W,\fs_{M}\cup \fs_{W})$ from a pairing between $\Bafu(M,\fs_{M})$ and $\Bafu(W,\fs_{W})$. Putting these results together, we obtain the gluing formula that expresses the Seiberg-Witten invariant in terms of cobordism induced map defined using relative Bauer-Furuta invariants. (See  \cite[Proposition 3.6.1]{KronheimerMonopoles}.) Concretely, that means 
\[
\begin{split}
\langle \overrightarrow{HM}^*(M,\fs_{M})(\alpha),[\Pic(M,\fs_{M})]\rangle=&\langle \overrightarrow{HM}^*(M\cup W,\fs_{M}\cup \fs_{W})(1),[\Pic(M,\fs_{M})]\rangle\\=& \operatorname{SW}(M\cup W, \fs_{M}\cup \fs_{W})\\
=&1.    
\end{split}
\]
This completes the proof.
\end{proof}
